D2.2 White-box methodologies, programming abstractions and libraries

This deliverable reports the results of white-box methodologies and early results of the first prototype of libraries and programming abstractions as available by project month 18 by Work Package 2 (WP2). It reports i) the latest results of Task 2.2 on white-box methodologies, programming abstractions and libraries for developing energy-efficient data structures and algorithms and ii) the improved results of Task 2.1 on investigating and modeling the trade-off between energy and performance of concurrent data structures and algorithms. The work has been conducted on two main EXCESS platforms: Intel platforms with recent Intel multicore CPUs and Movidius Myriad1 platform. Regarding white-box methodologies, we have devised new relaxed cache-oblivious models and proposed a new power model for Myriad1 platform and an energy model for lock-free queues on CPU platforms. For Myriad1 platform, the im- proved model now considers both computation and data movement cost as well as architecture and application properties. The model has been evaluated with a set of micro-benchmarks and application benchmarks. For Intel platforms, we have generalized the model for concurrent queues on CPU platforms to offer more flexibility according to the workers calling the data structure (parallel section sizes of enqueuers and dequeuers are decoupled). Regarding programming abstractions and libraries, we have continued investigat- ing the trade-offs between energy consumption and performance of data structures such as concurrent queues and concurrent search trees based on the early results of Task 2.1.The preliminary results show that our concurrent trees are faster and more energy efficient than the state-of-the-art on commodity HPC and embedded platforms.

==> Concurrent-Search-Trees.tex <==
% START SECTION
\subsection{Concurrent Search Trees}

We have developed the concurrent search tree libraries package that contains the following components:
\begin{enumerate}
  \item Non-blocking binary search tree (NBBST) (Section \ref{sec:NBBST})
  \item STM-based search trees (Section \ref{sec:STMbased})
  \begin{enumerate}
    \item Red-black tree (RBtree)
    \item AVL tree (AVLtree)
    \item Speculation-friendly tree based on the AVL tree (SFtree)
  \end{enumerate}
  \item Concurrent B-tree (CBtree) (Section \ref{sec:CBTree})
  \item Static cache-oblivious tree using the static vEB layout (VTMtree) (Section \ref{sec:VTMTree})
  \item DeltaTree ($\Delta$Tree) (Section \ref{sec:DeltaTree})
  \item Balanced $\Delta$Tree (b$\Delta$Tree) (Section \ref{sec:bDeltaTree})
  \item Heterogeneous $\Delta$Tree (h$\Delta$Tree) (Section \ref{sec:hDeltaTree})

\end{enumerate}

\paragraph{Obtaining and compilation.} Each of the libraries is provided in a separate repository 
for easy access and maintenance. A makefile for each of the library is also provided to aid compilations.
These libraries have been tested on Linux and Mac OS X platforms.

\paragraph{Running and outputs.} By default, the provided makefile will build the standalone benchmark 
version of the libraries which will accept these following parameters:

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
   \texttt{-r <NUM>    : Allowable range for each element (0..NUM)\\
-u <0..100> : Update ratio. 0 = Only search; 100 = Only updates\\
-i <NUM>    : Initial tree size (initial pre-filled element count)\\
-t <NUM>    : DeltaNode ($\UB$) size (ONLY USED IN DELTATREE FAMILIES)\\
-n <NUM>    : Number of benchmark threads\\
-s <NUM>    : Random seed. (0 = using time as seed, Default)
}}}
\\
\\
The benchmark outputs are formatted in this sequence: 

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
    \texttt{
0: range, insert ratio, delete ratio, \#threads, \#attempted insert, \#attempted delete, \#attempted search, \#effective insert, \#effective delete, \#effective search, time (in msec.)
}}}

Below is an example of DeltaTree usage:

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
\ttfamily
\$ ./DeltaTree -h \newline
DeltaTree v0.1\newline
===============\newline
Use -h switch for help.\newline
\newline
Accepted parameters\newline
-r <NUM>    : Range size\newline
-u <0..100> : Update ratio. 0 = Only search; 100 = Only updates\newline
-i <NUM>    : Initial tree size (inital pre-filled element count)\newline
-t <NUM>    : DeltaNode size\newline
-n <NUM>    : Number of threads\newline
-s <NUM>    : Random seed. 0 = using time as seed\newline
-d <0..1>   : Density (in float)\newline
-v <0 or 1> : Valgrind mode (less stats). 0 = False; 1 = True\newline
-h          : This help\newline
\newline
Benchmark output format: \newline
"0: range, insert ratio, delete ratio, \#threads, attempted insert, attempted delete, attempted search, effective insert, effective delete, effective search, time (in msec)"
}}

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
\ttfamily
\$ ./DeltaTree -r 5000000 -u 10 -i 1024000 -n 10 -s 0\newline
DeltaTree v0.1\newline
===============\newline
Use -h switch for help.\newline
\newline
Parameters:\newline
- Range size r:		 5000000\newline
- DeltaNode size t:	 127\newline
- Update rate u:	 10\% \newline
- Number of threads n:	 10\newline
- Initial tree size i:	 1024000\newline
- Random seed s:	 0\newline
- Density d:		 0.500000\newline
- Valgrind mode v:	 0\newline
\newline
Finished building initial DeltaTree\newline
The node size is: 25 bytes\newline
Now pre-filling 1024000 random elements...\newline
...Done!\newline
\newline
Finished init a DeltaTree using DeltaNode size 127, with initial 1024000 members\newline
\#TS: 1421050928, 511389\newline
Starting benchmark...\newline
Pinning to core 0... Success\newline
Pinning to core 3... Success\newline
Pinning to core 1... Success\newline
Pinning to core 8... Success\newline
Pinning to core 9... Success\newline
Pinning to core 10... Success\newline
Pinning to core 2... Success\newline
Pinning to core 11... Success\newline
Pinning to core 4... Success\newline
Pinning to core 12... Success\newline
\newline
0: 5000000, 5.00, 5.00, 10, 249410, 248857, 4501733, 195052, 53720, 1000568, 476\newline
\newline
Active (alloc'd) triangle:258187(266398), Min Depth:12, Max Depth:30 \newline
Node Count:1165332, Node Count(MAX): 1217838, Rebalance (Insert) Done: 234, Rebalance (Delete) Done: 0, Merging Done: 1\newline
Insert Count:195052, Delete Count:53720, Failed Insert:54358, Failed Delete:195137 \newline
Entering top: 0, Waiting at the top:0
}}

\paragraph{Pluggable library.} To use any component as a library, each libraries provides a (.h) header file and a simple, 
uniform API in C. These available and callable APIs are:

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
\textsc{Structure:}\\
\\
\texttt{<libname>\_t} : Structure variable declaration.\\
\\
\textsc{Functions:}\\
\\
\texttt{<libname>\_t* <libname>\_alloc()} :	Function to allocate the defined structure, returns the allocated (empty) structure.\\
\\
\texttt{void* <libname>\_free(<libname>\_t* map)} :	Function to release all memory used by the structure, returns NULL if succeed.\\
\\
\texttt{int <libname>\_insert(<libname>\_t* map, void* key, void* data)} : Function to insert a key and a linked pointer (data), returns 1 if succeed and 0 otherwise.\\
\\
\texttt{int <libname>\_contains(<libname>\_t* map, void* key)} : Function to check whether a key is available in the structure, returns 1 if yes and 0 otherwise.\\
\\
\texttt{void *<libname>\_get(<libname>\_t* map, void* key)} : Function to get the linked data given its key, returns the pointer of the data of the corresponding key and 0 if the 
key is not found.\\
\\
\texttt{int <libname>\_delete(<libname>\_t* map, void* key)} : Function to delete an element matches the given key, returns 1 if succeed and 0 otherwise. 
}}

As an example, the concurrent B-tree library provides the \texttt{cbtree.h} file that can be linked into
any C source code and provides the callable \texttt{cbtree\_t* cbtree\_alloc()} function. It is also possible
to use the MAP selector header (\texttt{map\_select.h}) plus defining which tree type to use 
so that  MAP\_\textless{operator}\textgreater functions instead is used instead as specific tree function as the below example:

\noindent\fbox{%
    \parbox{0.95\textwidth}{%
\ttfamily
\#define MAP\_USE\_CBTREE\newline
\#include "map\_select.h"\newline
\newline
int main ()\newline
\{\newline
 long numData = 10;\newline
 long i;\newline
 char *str;\newline
 \newline
 puts("Starting...");\newline
 \newline
 MAP\_T* cbtreePtr = MAP\_ALLOC(void, void);\newline
 assert(cbtreePtr);\newline
 \newline
 for (i = 0; i < numData; i++) \{\newline
     str = calloc(1, sizeof(char));\newline
     *str = 'a'+(i\%254);\newline
     MAP\_INSERT(cbtreePtr, i+1, str);\newline
 \} \newline
 for (i = 0; i < numData; i++) \{ \newline
     printf("\%ld: \%c\textbackslash{n}", i+1, *((char*)MAP\_FIND(cbtreePtr, i+1)));\newline
 \} \newline
 for (i = 0; i < numData; i++) \{ \newline
     printf("\%ld: \%d\textbackslash{n}", i+1, MAP\_CONTAINS(cbtreePtr, i+1));\newline
 \} \newline
 for (i = 0; i < numData; i++) \{ \newline
     MAP\_REMOVE(cbtreePtr, i+1);\newline
 \} \newline
 for (i = 0; i < numData; i++) \{ \newline
     printf("\%ld: \%d\textbackslash{n}", i+1, MAP\_CONTAINS(cbtreePtr, i+1));\newline
 \} \newline
 \newline
 MAP\_FREE(cbtreePtr);\newline
 puts("Done.");\newline
 return 0;\newline
\}
}}

\paragraph{Intel PCM integration.} All of the libraries provide support for Intel PCM measurement. 
To enable Intel PCM measurement metrics,
the compiler must be invoked using \texttt{-DUSE\_PCM} parameter during the libraries's compilation 
and all the Intel PCM compiled object files must be linked to the output executables.
  
\subsubsection{Non-blocking binary search tree} \label{sec:NBBST}
The Non-blocking binary search tree (NBBST) library contains the non-blocking binary search tree of Ellen \cite{EllenFRB10}.

\subsubsection{STM-based search trees} \label{sec:STMbased}
STM-based search trees library contains the Software Transactional Memory (STM)-based AVL tree (AVLtree), red-black tree (RBtree), and speculation
friendly tree (SFtree) from the Synchrobench benchmark \cite{synchrobench}.

\subsubsection{Concurrent Btree} \label{sec:CBTree}
Concurrent Btree (CBTree) library contains an optimized Lehman and Yao B-link tree \cite{Lehman:1981:ELC:319628.319663}. 
B-link tree is a highly-concurrent B-tree variant 
and it is still being used as a backend in popular database systems such as 
PostgreSQL\footnote{\url{https://github.com/postgres/postgres/blob/master/src/backend/access/nbtree/README}}.  

\subsubsection{Concurrent static vEB binary search tree}  \label{sec:VTMTree}
The Concurrent static vEB binary search tree (VTMTree) library contains a concurrent version of the static vEB binary search tree  \cite{BrodalFJ02} developed using GNU C Compiler v4.9.1's STM.

\subsubsection{DeltaTree ($\Delta$Tree)} \label{sec:DeltaTree}

Based on the new concurrency-aware vEB, we implement $\Delta$Tree \cite{deltatreeTR2013}, a practical, unbalanced, 
and pointer-based concurrent search tree. Figure \ref{fig:treeuniverse} illustrates a $\Delta$Tree $U$ which
is composed by a group of subtrees ($\Delta$Nodes).
A $\Delta$Node's internal nodes are put together in cache-oblivious
fashion using the concurrency-aware vEB layout (cf. Section \ref{sec:relaxed-veb}). The search operation for $\Delta$Tree
is wait-free. We are aware that the $\Delta$Tree has two major 
shortcomings, namely being unbalanced tree and has a
poor memory utilization because of the inter-node pointers usage.

In order to address the $\Delta$Tree shortcomings, we implement the Balanced $\Delta$Tree (b$\Delta$Tree).
b$\Delta$Tree is devised by improving the structure and the 
algorithm of $\Delta$Tree to support the concurrent, Btree-like bottom-up insertions, which
ensures balanced tree.
Another major change is that in b$\Delta$Tree, the fat-pointer $\Delta$Nodes are 
replaced with pointer-less $\Delta$Nodes. The removal of
$\Delta$Nodes internal pointers made way for 200\% more nodes to fit into the tree. The 
concurrent search operations supported by b$\Delta$Tree are still without locks and waits, but
they are no longer wait-free. Based on our study, a more-compact tree results in less data transfers.
And less data transfers leads to better performance and energy efficiency.

Finally, we implement the Heterogeneous $\Delta$Tree (h$\Delta$Tree), which is 
a better performing, more-compact tree than b$\Delta$Tree. h$\Delta$Tree is devised by changing
the leaf-oriented (external) tree layout of the leaf $\Delta$Nodes into an internal tree layout. 
This improvement allows 100\% more nodes to fit inside the tree, which further
improves the tree's overall operation performance.

Based on experimental insights, our $\Delta$Trees are different from previous theoretical designs of concurrent 
cache-oblivious (CO) trees such as the concurrent packed-memory CO tree and concurrent exponential CO tree \cite{BenderFGK05}. %BenderDF05, 
The concurrent packed-memory CO tree gives a good amortized memory transfer cost of $\Theta(\log_B N + (\log^2 N/B))$
for tree updates, assuming that operations occur {\em sequentially}. However, the proposed data representation 
requires each node to have the parent-child pointers. 
Besides the complication in re-arranging those pointers, we have found that eliminating pointers 
from the node to minimize memory footprint is significantly 
beneficial for cache-oblivious tree in practice (cf. improvement from $\Delta$Tree to b$\Delta$Tree in Section \ref{sec:bDeltaTree}). 
In the $\Delta$Tree experimental evaluation (cf. Section \ref{sec:evaluation}), b$\Delta$Tree
is 100\% faster than $\Delta$Tree in searching, which is attained by simply
removing pointers from the tree node.

In the concurrent exponential CO tree by Bender et al. \cite{BenderFGK05}, expected memory transfer cost
for search and update operations is $\mathcal{O}(\log_B N + (\log_\alpha \text{lg} N))$, assuming that all processors are {\em synchronous}. Cormen et al. \cite[pp. 212]{CormenSRL01}, however,  
wrote that although the underlying exponential tree algorithm is an important theoretical
breakthrough, it is complicated and unlikely to compete with similar sorting algorithms. 
In fact, nodes in the exponential tree grow exponentially in size, which not only complicates maintaining inter-node pointers but also exponentially increases the tree's memory footprint in practice. 
In contrast, the memory footprint of $\Delta$Tree with the fixed size $\Delta$Nodes gradually expands on-demand when the tree grows. Thanks to the fixed size $\Delta$Nodes, $\Delta$Tree exploits further locality by utilizing a "map" (cf. Section \ref{sec:mapdesc}) and an efficient inter-node connection (cf. Section \ref{sec:interdesc}).


\begin{figure}[!t] \centering \includegraphics[width=0.8\textwidth]{tree1}
\caption{Depiction of a $\Delta$Tree $U$. Triangles $T_x$ represent the $\Delta$Nodes.}
\label{fig:treeuniverse}
\end{figure}

\begin{figure}[!t] 
\centering 
\begin{algorithmic}[1] 
\Start{\textsc{node} $n$} \label{lst:line:nodestruct}
	\START{member fields:}
\State $tid \in \mathbb{N}$, if $> 0$ indicates the node is \textit{root} of a \par
	\hskip\algorithmicindent $\Delta$Node with an id of $tid$ ($T_{tid}$) 
\State $value \in
	\mathbb{N}$, the node value, default is \textbf{empty} 
\State $mark \in \{true,false\}$, a value of \textbf{true} indicates a logically \par 
	\hskip\algorithmicindent deleted node
\State $left, right \in \mathbb{N}$, left and right child pointers 
\State $isleaf \in {true,false}$, indicates whether the \par 
	\hskip\algorithmicindent node is a leaf of a $\Delta$Node, default is \textbf{true} 	\label{lst:line:leafdefault}
\END \End

\Statex
\Start{\textsc{$\Delta$Node} $T$} \label{lst:line:deltanodestruct}
\START{member fields:}
\State $\mathit{nodes}$, a group of pre-allocated \textsc{node} $n$ $\{n_1,n_2,\ldots,n_{\UB}\}$
\State $\mathit{buffer}$, $\Delta$Node's buffer (pre-allocated array of \par 
	\hskip\algorithmicindent $b_1,b_2,\ldots,b_{\mathit{\#threads}}$)
\END \End

\Statex
\Start{\textsc{$\Delta$NodeMeta} $M$} \label{lst:line:trianglestruct}
\START{member fields:}
\State $\mathit{locked}$, indicates whether a $\Delta$Node is locked 
\State $\mathit{opcount}$, a counter for the active update operations 
\State $\mathit{root}$, pointer to the root node of the $\Delta$Node ($T_x.n_1$)
\State $\mathit{mirror}$, pointer to the root node of the $\Delta$Node's mirror  \par 
	\hskip\algorithmicindent($T_{x'}.n_1$)
\END \End

\Statex
\Start{\textsc{universe} $U$} 		\label{lst:line:universe}
	\START{member fields:}
\State $root$, pointer to the $root$ of the topmost $\Delta$Node ($T_1.root$) 
\END \End
\end{algorithmic}
\caption{$\Delta$Tree's data structures.} \label{lst:datastruct}
\end{figure}

The $\Delta$Tree consists of $|U|$ $\Delta$Nodes of fixed size $\UB$. Each of
the $\Delta$Node contains a \textit{leaf-oriented} binary search tree (BST) $T_i, i=1,
\dots,|U|$. The $\Delta$Tree $U$ provides the following operations: \textsc{insertNode($v, U$)}, 
which adds value $v$ to the set $U$, \textsc{deleteNode($v, U$)} 
for removing a value $v$ from the set, and
\textsc{searchNode($v, U$)}, for determining whether value $v$ exists in the
set. We use the term \textit{update} operation for either insert or delete
operation. We assume that duplicate values are not allowed inside the set and a
special value, for example $0$, is reserved as an indicator of an \textsc{Empty}
value.

\paragraph{Data structures.}

The implementation of $\Delta$Tree utilizes the data structure in
Figure \ref{lst:datastruct}. The topmost level of $\Delta$Tree is represented by
a struct \textsc{universe} (line \ref{lst:line:universe}) that contains 
a pointer (\textbf{root}) 
to the root node of the first $\Delta$Node ($T_1.n_1$).
A $\Delta$Tree is formed by a group of $\Delta$Nodes. 

$\Delta$Tree's $\Delta$Nodes are represented by the struct
\textsc{$\Delta$Node} (line \ref{lst:line:deltanodestruct}). A $\Delta$Node consists
of a collection of $\UB$ \textbf{nodes} and a \textbf{buffer} array. 
$\Delta$Node's \textbf{buffer} array length is equal 
to the number of operating threads. Each $\Delta$Node is accompanied by
a metadata \textsc{$\Delta$NodeMeta} that holds lock and counters variable.

Struct \textsc{$\Delta$NodeMeta} (line \ref{lst:line:trianglestruct})
acts as metadata for every $\Delta$Node.
This structure consists of a field \textbf{opcount}, which is a counter that indicates 
the number of insert/delete threads that
are currently operating within that $\Delta$Node; and field \textbf{locked} that indicates 
whether a $\Delta$Node is currently locked by a maintenance operation.
When \textbf{locked} is set as \textit{true}, no insert/delete threads 
are allowed to get into a $\Delta$Node. 
Lastly, \textsc{$\Delta$NodeMeta} contains \textbf{root} pointer 
that points to the first  \textsc{node}
of $\Delta$NodeMeta's accompanying $\Delta$Node, and the pointer \textbf{mirror} that points 
to the \textit{root} of the $\Delta$Node's mirror. 


Each \textsc{node} structure (line \ref{lst:line:nodestruct}) contains field \textbf{value}, 
which holds a value for guiding the search, or a data value if it resides in a leaf-node.
Field \textbf{mark} indicates a logically deleted value, if set to \textit{true}. 
A \textit{true} value of \textbf{isleaf} indicates the node is a leaf
node, and \textit{false} otherwise. Field \textbf{tid} is a unique
identifier of a corresponding $\Delta$Node and it is used to let a thread know whether it has moved
between $\Delta$Nodes. A \textbf{tid} is only defined in the root node of a $\Delta$Node.

\paragraph{$\Delta$Tree functions.}

% Searching Algorithm
\begin{figure}[!t] 
\centering \begin{algorithmic}[1] 

\Function{searchNode}{$v, U$}
\State $p \gets U.root$
\While{(TRUE)} 	\label{lst:line:search-while}
	\State $lastnode \gets p$	\Comment{atomic assignment} \label{lst:line:lastnode-p}
        \If{($p.value < v$)}		\label{lst:line:searchless}
            \State $p \gets p.left$
        \Else					\label{lst:line:searchelse}
            \State $p \gets p.right$ 
        \EndIf
        \If{($!p$ \textbf{or} $lastnode.isleaf =$ TRUE)}	\label{lst:line:searchifleaf}
        		\State \textbf{break} 					 \label{lst:line:search-end}
	\EndIf
\EndWhile
\If{($lastnode.value = v$)} 		\label{lst:line:linsearch3}
	\If{($lastnode.mark =$ FALSE)}	 \Comment{lastnode is not deleted}	\label{lst:line:linsearch1}
		\State\Return TRUE 
	\Else 
		\State\Return FALSE 
	\EndIf 
\Else \State \{Search the last visited $\Delta$Node's \textit{buffer} for $v$\}	\label{lst:line:searchbuffer}
	\If{(\{$v$ is found\})}							\label{lst:line:linsearch2}
		\State\Return TRUE 
	\Else 
		\State\Return FALSE 
	\EndIf 
\EndIf 
\EndFunction
\end{algorithmic}
\caption{$\Delta$Tree's \textit{wait-free} search algorithm.}\label{lst:nodeSearch}
\end{figure}

$\Delta$Tree provides basic functions such as search, insert and delete functions. 
We refer insert and delete operations
as the \textit{update} operations.

Function \textsc{searchNode($v,U$)} (cf. Figure \ref{lst:nodeSearch}), is going to walk 
over the $\Delta$Tree to
find whether the value $v$ exists in $U$ (Figure \ref{lst:nodeSearch}, lines \ref{lst:line:lastnode-p}--\ref{lst:line:search-end}). 
The  \textsc{searchNode($v,U$)} function returns \textbf{true} whenever $v$ has been
found, or \textbf{false} otherwise (Figure \ref{lst:nodeSearch}, line \ref{lst:line:linsearch1}). 
This operation is
guaranteed to be wait-free (cf. Lemma \ref{lem:waitfreesearch}).

\begin{lemma} \label{lem:waitfreesearch}
$\Delta$Tree search operation is \textit{wait-free}.
\end{lemma}
\begin{proof}(Sketch) The proof can be served based on these observations on Figure \ref{lst:nodeSearch}:
\begin{enumerate}
\item \textsc{SearchNode} and invoked \textsc{SearchBuffer} (line \ref{lst:line:searchbuffer}) do not wait for any locks.
\item The number of iterations in the \textit{while} loop (line \ref{lst:line:search-while})
	 is bounded by the \textit{height}  $T$ of the tree, or $\mathcal{O}(T)$. The loop is always ended
	 whenever a leaf node or an empty node is found in line \ref{lst:line:search-end}.
\item \textsc{SearchBuffer} time complexity is bounded by the buffer size, which is a constant.
\end{enumerate}
Therefore the  \textsc{SearchNode} time is bounded by $\mathcal{O}(T)$, where $T$ is the height of the tree.
\end{proof}


\begin{figure*}[!t]
\centering
\scriptsize
\begin{minipage}[!t]{0.47\linewidth}
\begin{algorithmic}[1]


%Delete Helper Algorithms
\Function{deleteNode}{$v, p$}		\label{lst2:line:deletefunc}				

\State $p \gets U.root$
\State \textit{BEGIN}:
\If{(\{Entering new $\Delta$Node $T_x$\})}                 			                                                 
   \State  Decrement previous $\Delta$Node's opcount ($T'_x.opcount$)				
   \State  Wait if $\Delta$Node is currently maintained 		\label{lst2:line:waitdelete}
\EndIf

\If{Is at leaf ($p.isleaf =$ TRUE)) \textbf{or} at the tree's last level node}
        \If{($p.value = v$)}
            \If{(\textsc{CAS}($p.mark$, FALSE, TRUE) != FALSE))}              	\label{lst2:line:markdel}       
                	\State Decrement  $T_x.opcount$	                                      \Comment{$v$ is already deleted}
            \Else	
             	\If{$p$ is still the leaf node} 	\label{lst2:line:markdel-check}
			\If{(\textsc{TAS}($T_x.locked$))} \Comment{Acquire the maintenance lock} \label{lst2:line:lockbuf-del}
				\State Decrement $T_x.opcount$	\label{lst2:line:dec-opcount-del}
				\State Wait for all updates to finish ($T_x.opcount$=0) \label{lst2:line:spinwait-main-del} 
                			\State Do node merge if needed \label{lst2:line:merge}          
			\EndIf       
		\Else		 
			\State Re-try delete from current node $p$ \label{lst2:line:retrydel}
		\EndIf
            \EndIf
        \Else
        		\State Search ($T_{x}.\mathit{buffer}$) for $v$
	   	\If{$v$ is found in $T_{x}.\mathit{buffer.idx}$}
                 	\State Remove $v$ from $T_{x}.\mathit{buffer.idx}$	\label{lst2:line:bufdel} 	\Comment{buffered delete}
	    	\EndIf
		\State Decrement $T_x.opcount$                                            
    	\EndIf
\Else 
	\If{($v < p.value$)}
        		\State Go to left child ($p \gets p.left$)
	\Else
        		\State Go to right child  ($p \gets p.right$)
	\EndIf	
	\State Restart from \textit{BEGIN}
\EndIf
\EndFunction

\State

%Insert Helper Algorithms
\Function{insertNode}{$v, p$}	\label{lst2:line:insertfunc}
\State $p \gets U.root$

\State \textit{BEGIN}:

\If{(\{Entering new $\Delta$Node $T_x$\})}                 			                                                 
   \State  Decrement previous $\Delta$Node's opcount ($T'_x.opcount$)				
   \State  Wait if $\Delta$Node is currently maintained 		\label{lst2:line:waitinsert}
\EndIf

\algstore{bkbreak}
\end{algorithmic}
\end{minipage}
\qquad
\begin{minipage}[!t]{0.47\linewidth}
\begin{algorithmic}[1]

\algrestore{bkbreak}
    
\If{Not at the tree's last level node}                                                    
        \If{($v < p.value$)}                                                                              
            \If{Is at leaf ($p.isleaf =$ TRUE)}  									                              
                \If{(CAS($p.left.value$, \textbf{empty}, $v$) = \textbf{empty})}       \label{lst2:line:ins-lp1} 	\label{lst2:line:growins1}    
                	   \State Do insert to the left   	                          \label{lst2:line:growins1-end}                         
                   \State Decrement $T_x.opcount$ 
                \Else
                    \State Re-try insert from $p$ 		\label{lst2:line:retryinsleft}                    
                \EndIf
            \Else
                \State Go to left child ($p \gets p.left$) ) and restart from \textit{BEGIN}     
            \EndIf
        \ElsIf {($v > p.value$)}                                                                      
            \If{(Is at leaf ($p.isleaf =$ TRUE)}                                 
                \If{(CAS($p.left.value$, $\textbf{empty}$, $p.value$) = \textbf{empty})}  \label{lst2:line:ins-lp2}  \label{lst2:line:growins2} 
                	   \State Do insert to the right                    
	   	   \State Decrement $T_x.opcount$ 
                \Else
                    \State Re-try insert from $p$  \label{lst2:line:retryinsright}             
                \EndIf
            \Else
                \State  Go to right child ($p \gets p.right$) and restart from \textit{BEGIN}             	\label{lst2:line:right-end}
             \EndIf
        \ElsIf {($v = p.value$)}                                                                                            
            \If{Is at leaf ($p.isleaf =$ TRUE)}                                   
                \If{$v$ is not deleted ($p.mark =$ FALSE)}								
                    \State Decrement $T_x.opcount$                            \Comment{$v$ already exist} \label{lst2:line:valexist}
                \Else
                	   \State Do insert right
                \EndIf
            \Else
                \State Go to right child ($p \gets p.right$) and restart from \textit{BEGIN}       
            \EndIf
        \EndIf
\Else			
		\If{$v$ is already in $T_x.\mathit{buffer}$}
			\State Decrement $T_x.opcount$
		\Else
			\State Put $v$ inside $T_x.\mathit{buffer}$ \label{lst2:line:insertbuffer}		\Comment{buffered insert}	
			\If{(\textsc{TAS}($T_x.locked$))} \Comment{Acquire maintenance lock} \label{lst2:line:lockbuf}
			\State Decrement $T_x.opcount$ \label{lst2:line:dec-opcount}
			\State Wait for all updates to finish ($T_x.opcount$=0)  \label{lst2:line:spinwait-main}
			\State do \textsc{rebalance}($T_x$) or \textsc{expand($p$)}  \label{lst2:line:expand}
			\EndIf 
		\EndIf
\EndIf
\EndFunction
\end{algorithmic}
\end{minipage}
\caption{$\Delta$Tree's concurrent update (\textit{insert} and \textit{delete}) algorithms.}
\label{lst:pseudo-ops-simple}
\end{figure*}

Function \textsc{insertNode($v, U$)} (cf. Figure \ref{lst:pseudo-ops-simple}, line \ref{lst2:line:insertfunc}) 
inserts value $v$ at a leaf of $\Delta$Tree, 
provided $v$ does not exist in the
tree (Figure \ref{lst:pseudo-ops-simple}, line \ref{lst2:line:valexist}). 
Following the nature of a leaf-oriented tree, a successful insert operation 
replaces a leaf with a subtree of three nodes \cite{EllenFRB10} (cf. Figure
\ref{fig:treetransform}a and in Figure \ref{lst:pseudo-ops-simple}, 
lines \ref{lst2:line:growins1} and \ref{lst2:line:growins2}). Because $\Delta$Tree
structure is pre-allocated, an insert operation needs only to do a "logical" replacement, or 
only replacing the value of a leaf and its children.

\begin{figure}[!t] \centering \includegraphics[scale=0.8]{tree2}
\caption{(a)\textit{Rebalancing}, (b)\textit{Expanding}, and (c)\textit{Merging} operations on $\Delta$Tree.}
\label{fig:treetransform}
\end{figure}

The function \textsc{deleteNode($v, U$)} (cf. Figure \ref{lst:pseudo-ops-simple}, line \ref{lst2:line:deletefunc}) 
{\em marks} the leaf that contains value $v$ as deleted. \textsc{deleteNode($v, U$)} fails if $v$ does not exist in the tree or 
the leaf containing $v$ is already mark as deleted. 

\textsc{insertNode} and \textsc{deleteNode} operations are non-blocking 
to other \textsc{searchNode, insertNode} and \textsc{deleteNode} operations.
%(cf. Lemma \ref{lem:linear-search} and \ref{lem:nonblock-update}).
Both of the update operations are using the single word CAS (Compare and Swap)
and \textit{leaf-checking} to provide linearizability between the
operations (cf. Figure \ref{lst:pseudo-ops-simple}, lines \ref{lst2:line:markdel} and 
\ref{lst2:line:markdel-check} for delete, and \ref{lst2:line:ins-lp1}
and \ref{lst2:line:ins-lp2} for insert). 

\subparagraph{Maintenance functions.} \label{sec:maintenance-func}

Other than the basic functions, $\Delta$Tree has tree maintenance functions 
that are invoked in certain cases of inserting and deleting a node from the tree. 
These functions, namely rebalance, expand and merge, are the unique
feature of $\Delta$Tree that acts as a garbage collectors for marked nodes 
and as a safeguard to maintain $\Delta$Tree's small height.

Function \textsc{rebalance($T_v.root$)} (cf.  Figure \ref{lst:pseudo-ops-simple} 
line \ref{lst2:line:expand}) is responsible for rebalancing a
$\Delta$Node after an insertion.
Figure \ref{fig:treetransform}a illustrates the rebalance operation. If a
new node $v$ is to be inserted at the last level $H$ of $\Delta$Node $T_1$, the
$\Delta$Node is rebalanced to a complete BST. All
leaves' height are then set to $\lfloor\log N\rfloor + 1$,
where $N$ is the number of leaves (e.g., $a,v,x,z$ in Figure \ref{fig:treetransform}a). 
In the same Figure \ref{fig:treetransform}a, after rebalance, tree $T_1$ height reduces from 4 to 3.

We also define \textsc{expand($l$)} function (cf.  Figure \ref{lst:pseudo-ops-simple} 
line \ref{lst2:line:expand}) that is responsible for
creating a new $\Delta$Node and connecting it to the parent of a leaf node $l$ 
(cf. Figure \ref{fig:treetransform}b).
Expanding is triggered only if 1) after \textsc{insertNode($v, U$)}, leaf that contains 
$v$
will be at the last level of a $\Delta$Node; and 2) rebalancing will no longer
reduce the current height of $\Delta$Node $T_i$. 
For example if an expand takes place at node $l$ which is located at the lowest
level of a $\Delta$Node, or $depth(l) = H$, 
the parent of $l$ swaps one of its child pointer that previously points to
$l$ into the root of the newly created $\Delta$Node's $root$ (cf. Figure \ref{fig:treetransform}b).

Function \textsc{merge($T_x.root$)} (cf.  Figure \ref{lst:pseudo-ops-simple} 
line \ref{lst2:line:merge}) is defined to merge $T_x$ with its sibling. 
For example in Figure \ref{fig:treetransform}c, $T_2$ is
merged into $T_3$. Then
the pointer of $T_3$'s grandparent that previously points
to the parent of both $T_3$ and $T_2$ is replaced by a pointer to $T_3$.
Merge operation is invoked provided that in a particular $\Delta$Node, where 
a deletion has taken place, is filled less than $2^{^t/_2}$ of its capacity 
(where $t = \log(\UB)$) and both
nodes of that $\Delta$Node and its siblings are going to fit into a single $\Delta$Node. 

Before any maintenance operation starts, the threads responsible 
are required to do Test and Set (TAS) on $\Delta$Node's \textit{locked} 
field (cf. Figure \ref{lst:pseudo-ops-simple}, lines \ref{lst2:line:lockbuf} and  \ref{lst2:line:lockbuf-del}).
If a $\Delta$Node's \textit{locked} has been set to TRUE,
new incoming update operations are forced to wait at the tip of that $\Delta$Node
so that they will not interfere with the maintenance operation  
(cf. Figure \ref{lst:pseudo-ops-simple}, line \ref{lst2:line:waitdelete}
and \ref{lst2:line:waitinsert}) . 

For efficiency, a $\Delta$Node's maintenance operation starts 
after a batch of concurrent update operations within that $\Delta$Node. The TAS
also serves as a mechanism to make the concurrent update operations compete for 
a maintenance lock (\textit{locked} variable). The losing threads will
leave their maintenance burden 
to a thread who successfully acquired the $\Delta$Node's \textit{locked} variable.

After the maintenance operation finished, $\Delta$Node's \textit{locked} 
is released by the maintenance thread. 
Therefore, waiting update threads can continue with their respective operation 
within the newly-maintained $\Delta$Node.

Note that although \textsc{rebalance}
and \textsc{merge} execution are sequential within a $\Delta$Node, invoking 
these functions involves at most $2\times\UB$ nodes, where a constant $\UB \ll N$.
Section \ref{sec:diff-UB} discuss on the effect of different $\UB$ values to the 
$\Delta$Tree's search and insert performance.

\paragraph{Mirroring.} \label{sec:mirroring}
Whenever a $\Delta$Node is undergoing a
maintenance operation (balancing, expanding, or merging), a mirroring operation
also takes place to facilitate the wait-free search. 
Mirroring works by maintaining the original $\Delta$Node and writing 
the results into the mirror $\Delta$Node. 

After a maintenance operation finishes, the pointer to the root of the maintained $\Delta$Node 
is switched to the root of the $\Delta$Node's mirror. In result, the mirror, or maintained $\Delta$Node, 
is now becomes part 
of $\Delta$Tree, replacing the "old" $\Delta$Node. As the $\Delta$Node's buffer is enclosed within a $\Delta$Node, 
it is also switched at the same time $\Delta$Node was switched. 
As a result, the original $\Delta$Node and its helping buffer served as the latest snapshot, which
enables wait-free search for $\Delta$Tree. 

\subsubsection{Balanced $\Delta$Tree}\label{sec:bDeltaTree} 

$\Delta$Tree served as a proof of concept
of a concurrency-aware vEB-based search trees, although it has major weaknesses that 
can affect its empirical performance.
First, the 
\textit{left} and \textit{right} pointers are occupying larger memory 
spaces compared to the data values. For example, in a $\Delta$Node 
with 127 nodes, the set of pointers will occupy 2032 bytes ($127 \times 16$ bytes) 
of memory in a 64-bit operating system. 
Therefore, the amount of space used by pointers alone 
is twice the amount of space used by the data values (i.e., $127 \times 4$ bytes = 1016 bytes, 
assuming node's $value$ is a 4 bytes integer).
This is inefficient, because every block transfer between any levels of memory carries
a bigger portion of pointers instead of important data.
Second, inserting a sequence of increasing or decreasing 
numbers into $\Delta$Tree will results a linked-list of $\Delta$Node (i.e., $\Delta$Tree's
height is equal to $N$, or the number of elements). This is a direct implication 
of the unbalanced form of $\Delta$Tree.  

Balanced $\Delta$Tree (b$\Delta$Tree) is implemented to address the $\Delta$Tree's weaknesses. 
b$\Delta$Tree is developed by devising three major
strategies, namely replacing internal $\Delta$Node pointers with map, crafting the
efficient inter-node connection, and ensures that the tree is always balanced.

Improving $\Delta$Tree to become a pointer-less concurrent cache-oblivious 
is difficult. For example, Brodal, et al. \cite{BrodalFJ02}
have discussed about pointer-less CO BST and their
implementation involves heavy calculation to determine the children positions of a node.
In contrast to our $\Delta$Tree that consists of group of $\Delta$Nodes, 
they are treating their tree as $N$-sized vEB-layout tree. Thus, not only we need 
to address the node parent-child pointers, we must also consider the inter-$\Delta$Node pointers. 

As the matter of fact, having a fixed-sized $\Delta$Nodes ($\UB \ll N$) is 
actually advantageous. A single pre-calculated
map of all $\UB$ nodes can be generated once and used by all operations 
throughout the 
whole tree. The inter-$\Delta$Node connection still need pointers
though, but instead of $2\times\UB$ pointers, we will show that 
a significant reduction of pointers ($^1/_2\times\UB$) is possible.

\paragraph{"Map" instead of pointers.}  \label{sec:mapdesc}
\begin{figure}[!t] \centering 
\begin{algorithmic}[1] 


\Start{\textbf{Map}} \label{lst:line:map}
	\START{member fields:}
\State $left \in
	\mathbb{N}$, interval of the \textit{left} child pointer address
\State $right \in
	\mathbb{N}$, interval of the \textit{right} child pointer address 
%\State $parent \in
%	\mathbb{N}$, interval of the \textit{parent} pointer address
\END \End

\Statex
\State \textbf{Map} $map[\UB]$

\Statex 

\Function{right}{p, base}  \label{lst:line:right}
    \State $nodesize \gets  \textsc{sizeOf}(\textbf{single node})$
    \State $idx \gets (p - base)/nodesize$
    
    \If {($map[idx].right$ != 0)}
        \State \Return $base + map[idx].right$
    \Else
        \State \Return 0
    \EndIf
\EndFunction

\Statex 

\Function{left}{p, base} \label{lst:line:left}
    \State $nodesize \gets  \textsc{sizeOf}(\textbf{single node})$
    \State $idx \gets (p - base)/nodesize$
    
    \If {($map[idx].left$ != 0)}
        \State \Return $base + map[idx].left$
    \Else
        \State \Return 0
    \EndIf
\EndFunction
\end{algorithmic}
\caption{\textit{Mapping} functions.}
\label{lst:map-func}
\end{figure}

The Balanced $\Delta$Tree is implemented 
by completely eliminating (\textit{left} and \textit{right}) 
pointers within a $\Delta$Node. Instead, these pointers are replaced with the corresponding
\textsc{left} and \textsc{right} functions (Figure \ref{lst:map-func}, lines  \ref{lst:line:right}
and \ref{lst:line:left}). \textsc{left} and \textsc{right} functions, given an arbitrary node $v$ and
the root memory address of its container $\Delta$Node, will return the the addresses 
of the left and right child nodes of $v$. These functions will return $0$ if $v$ is the deepest node
within a $\Delta$Node. The \textsc{left} and \textsc{right} functions requires 
a \textit{map} array with $\UB$ length to determine a node's children address (Figure  \ref{lst:map-func}, line  \ref{lst:line:map}).

$\Delta$Node's \textit{map} is a read-only record of the nodes' memory address differences.
The address differences of every $\Delta$Node's nodes and its left and right children 
are pre-calculated and recorded when the Balanced $\Delta$Tree is initialized. 
Because $\Delta$Nodes are using the same fixed-size concurrency-aware vEB layout, 
only one map is needed for all of the available $\Delta$Nodes.  
Therefore, since only one \textit{map} with size
$\UB$ is used for all traversing, memory footprint for the Balanced $\Delta$Tree's 
$\Delta$Node operations can be kept minimum (namely, the read-only map is always cached). 
Please note that the \textit{map} only supports internal (within $\Delta$Node) node traversal. 

\paragraph{Inter-$\Delta$Node connection.}  \label{sec:interdesc}

To facilitate the traversing from one $\Delta$Node to another, the inter-$\Delta$Node connection
mechanism is used in addition to the \textit{map}.
To use the inter-$\Delta$Node connection, first we logically assign color to each of the $\Delta$Node's
node edge. 
Each node has only two outgoing edges, which are the left edge and the right edge. 
These left and right edges are assigned 0 and 1 color, respectively.
Now any paths traversed from the $root$ of a $\Delta$Node to reach 
any internal node will produce a bit-sequence of colors. This bit representation
can be translated into an array index that contains a pointer to a child $\Delta$Node. 
The maximum size of the bit representation is the height of $\Delta$Node or $\log(\UB)$ bits.
We are using leaf-oriented tree and allocate a pointer array with
$^1/_2\times\UB$ length. Pseudocode in Figure \ref {lst:scannode-func}
explains how the inter-$\Delta$Node connection works in a pointer-less search function.

The removal of the internal nodes' pointers results in 200\% more
node counts in a $\Delta$Node compared to the $\Delta$Tree with the same $\UB$ size.
A $\Delta$Node's struct is now consist of internal nodes, which is just an array of keys, 
plus an array of $^1/_2\times\UB$ pointers for the inter-$\Delta$Node connection.

\begin{figure}[!t] \centering 
\begin{algorithmic}[1] 

\Function{pointerLessSearch}{key, $\Delta$Node, maxDepth}
    
  \While{$\Delta$Node is not leaf}
   	\State $bits \gets 0$
    	\State $depth \gets 0$
   	\State $p \gets {\Delta}Node.root$
   	\State $base \gets p$
    	\State $link \gets {\Delta}Node.link$
    
    	\While{($p \And p.value$ != EMPTY)}  \Comment{continue until leaf node} 
        		\State $depth \gets depth + 1$ \Comment{increment depth}
        		\State $bits \gets bits << 1$ \Comment{shift one bit to the left in each level}
        		\If {($key < p.value$)}
             		\State $p \gets$ \textsc{left}($p, base$)
        		\Else
            		\State $p \gets$ \textsc{right}($p, base$)
            		\State $bits \gets bits+1$ \Comment{right child color is 1}
        		\EndIf
    	\EndWhile
    	%\State $bits \gets bits >> 1$
	\LComment{pad the $bits$ to get the index of the child $\Delta$Node's pointer:}
    	\State $bits \gets bits << (maxDepth - depth) - 1$ 
    	\LComment{follow nextRight if highKey is less than searched value:}
    	\If{(${\Delta}Node.highKey <= key$)}
     		\State ${\Delta}Node \gets {\Delta}Node.nextRight$
   	\Else
     		\State ${\Delta}Node \gets link[bits]$ \Comment{jump to child $\Delta$Node}
   	\EndIf
  \EndWhile
  \State \Return ${\Delta}Node$
\EndFunction

\end{algorithmic}
\caption{Search within pointer-less $\Delta$Node. This function will return the {\em leaf} $\Delta$Node containing
the searched key. From there, a simple binary search using \textsc{left} and \textsc{right} functions
is adequate to pinpoint the key location. The search operations are utilizing both the 
$nextRight$ pointers and  $highKey$
variables to handle concurrent $\Delta$Node splitting~\cite{Lehman:1981:ELC:319628.319663}.}
\label{lst:scannode-func}
\end{figure}

\paragraph{Concurrent and balanced tree.}

%We improve the structure the $\Delta$Tree and the 
%We replace the array nodes in B-link trees with the concurrency-aware vEB layout $\Delta$Nodes.
To enable both of the concurrency and balanced tree out of the $\Delta$Tree, 
new variables are added into the $\Delta$Nodes and
changes are made to the $\Delta$Tree's update and maintenance operations.
We improved $\Delta$Tree's update algorithms by adopting 
the algorithms from the concurrent lock-based 
B-link trees \cite{Lehman:1981:ELC:319628.319663} 
by Lehman and Yao.

The insert operations in b$\Delta$Trees are now done in a bottom-up fashion 
to ensure that the tree is always balanced.
Meanwhile, the search operations are done in a top-down, left-to-right fashion.

The modification to how the insert and search operations work results in the omission
of both \textsc{merge($T_x.root$)} and \textsc{expand($l$)} functions 
(cf. Section \ref{sec:maintenance-func}). 
Instead, the new \textsc{split($T_v$)} functions is introduced to aid the bottom-up
tree building.

\textsc{split($T_v$)} functions splits the $\Delta$Node $T_v$ into $T'_v$ and 
a right sibling $T_x$. The internal nodes that were previously occupying 
$T_v$ are distributed evenly between $T'_v$ and $T_x$. 
If $T_v$ is the topmost $\Delta$Node, a new parent $\Delta$Node $T_p$ is created as well, taking
both $T'_v$ and $T_x$ as its children. 
The split operation concludes with an insertion of the lowest value from $T_x$ nodes
into $T_p$.
The $\Delta$Node split is triggered only when a $\Delta$Node overflows after an insertion, 
which means it is at least filled with ($2^{^t/_2}$) internal nodes, where $t=\log(\UB)$.

Beside the addition of split operation, 
two additional variables are added inside the struct \textsc{$\Delta$NodeMeta}. 
These additional variables 
are $nextRight$ pointer, which points to the right sibling $\Delta$Node; and $highKey$
variable that contains the upper-bound value of the $\Delta$Node. Starting with NULL values,
both of these new variables are populated when the $\Delta$Node splits. For example, 
after $T_v$ splits, the $T_v.nextRight$ is going to point to $T_x$, 
while $T_v.highKey$ is set to the minimum value of all the
nodes in $T_x$. These new variables
help the concurrent search with respect to the node splits \cite{Lehman:1981:ELC:319628.319663}.

With the addition of $nextRight$ and $highKey$ variables, 
Balanced $\Delta$Tree's search operations do not need locks and waits
(cf. Figure \ref{lst:scannode-func}). However, 
the search cannot be regarded as wait-free. 
According to Lehman and Yao \cite{Lehman:1981:ELC:319628.319663}, 
in the worst case, which is extremely unlikely, an infinite loop caused by 
continuous $\Delta$Node splits might happen.

To address the memory wastage, 
the same rebalancing procedure as in Figure \ref{fig:treetransform}a is employed by b$\Delta$Tree. 
The rebalancing also helps
to clean-up the nodes marked for deletion, keeping $\Delta$Nodes always in a good shape.
A mirroring whenever the tree splits and rebalances are also retained to make the tree
traversals do not require any locks and waits. 

\subsubsection{Heterogeneous $\Delta$Tree}\label{sec:hDeltaTree}
 
In Balanced $\Delta$Tree, the leaf-oriented (or external tree) layout is 
adopted for $\Delta$Nodes in order to facilitate the inter-$\Delta$Node connection mechanism
using $^1/_2\times\UB$ pointers.
However, it is not necessary for the leaf $\Delta$Nodes to have leaf-oriented 
layout since they do not have any successor $\Delta$Nodes.
 
Based on the above observation, we devise a heterogeneous balanced 
$\Delta$Tree by changing the layout of the balanced $\Delta$Tree's leaf $\Delta$Nodes.
This new layout uses internal tree instead of the external tree for the leaf $\Delta$Nodes. 
With this layout change, 100\% more key nodes are now fit into any leaf $\Delta$Node,
if compared to the previously non-leaf $\Delta$Nodes with the same $\UB$ limit.
To save more memory spaces, we also remove the array of pointers for intra-$\Delta$Node connection
in the leaf $\Delta$Nodes metadata. 

With this improved version of $\Delta$Tree, or heterogeneous $\Delta$Tree, we find that the efficiency of 
searches is improved. Compared to $\Delta$Tree and balanced $\Delta$Tree, the heterogeneous $\Delta$Tree
delivers lower number of cache misses and more efficient branching.

\subsection{Energy Consumption Analysis of Concurrent Search Trees} \label{sec:evaluation}
We have evaluated our conceptual ideas of concurrency-aware vEB by experimentally analyzing the performance and energy efficiency of $\Delta$Tree (Section \ref{sec:DeltaTree}), 
balanced $\Delta$Tree (b$\Delta$Tree) (Section \ref{sec:bDeltaTree}), and heterogeneous $\Delta$Tree
(h$\Delta$Tree) (Section \ref{sec:hDeltaTree}) in comparison with that of the prominent concurrent search trees in the literature (cf. Section \ref{sec:benchsetup}). The experimental evaluation was conducted on both Intel high performance computing (HPC) platforms and an ARM embedded platform. 
We have also evaluated how $\Delta$Trees would perform using different $\UB$ values (cf. Section \ref{sec:diff-UB}) as well as in the worst-case and average-case setups against the highly optimized B-tree  and the widely used GCC's std::set (cf. Section \ref{sec:worstCase}).

\subsubsection{Testbed choices} \label{sec:benchsetup}

Pthreads were used for threading and all running threads were pinned to
the available physical cores using pthread\_setaffinity\_np. 
GCC 4.9.1 was used with -O2 for all program compilations. All of the tests
are repeated at least $10\times$ to guarantee consistent results.

Several decisions have been made for choosing VTMtree's size, $\Delta$Nodes' $\UB$
and CBTree's block size. Since the VTMtree's size was fixed, 
we set it to $2^{23}$ so that VTMtree needed not to expand. For fair
comparisons, $\Delta$Trees' $\UB$ and CBTree's 
order were set to their respective values so that each $\Delta$Node and CBTree's node fitted within a memory page (4KB).
Therefore, CBTree's order was set to 336.

\paragraph{Performance benchmark setup.}

Performance indicators (in operations/second) were calculated 
using the number of ($\mathit{rep}=\num[group-separator={,}]{5000000}$) operations 
divided by the maximum time for the threads to finish the whole operations.
Combination of
update rate $u=\{0, 20, 50\}$ and number of thread 
$\mathit{nr}=\{1, 2, \ldots, 16\}$ were used for each runs.
Update rate of 0 equals to 100\% search, 
while 50 update rate equals to 50\% insert and delete operations out of $\mathit{rep}$ operations.
All involved operations used random
values of $v \in (0, \mathit{init} \times 2], v \in \mathbb{N}$. 
All the trees were initialized with a number $init$ of nodes to simulate trees 
that partially fit into the last level cache (LLC) of the evaluating platform. 
The $init$ values were $\num[group-separator={,}]{4194303}$ and $\num[group-separator={,}]{2097151}$ for the Intel HPC platform and ARM embedded platform, respectively. 

The Intel HPC platform was equipped with 
dual Intel Xeon E5-2670 CPUs, 
with total of 16 cores (no hyperthreading). The platform had 32GB of RAM,  
2MB (8$\times$256KB) L2 cache, and shared 20MB L3 cache for each CPU. 
Linux with kernel version 2.6.32-358 was used in this platform.

The embedded ARM platform was a Samsung Exynos 5410
octa-core ARM board with ARM's big.LITTLE CPU. This board had four Cortex-A15 1.6Ghz cores 
and four Cortex-A7 1.2Ghz cores in a single CPU and 2GB LPDDR3 RAM. The A15 cores
had a 2MB shared L2 cache while the A7 cores had a 512KB shared L2 cache.
Although the CPU had a total of 8
cores, only 4 cores could be active at a time. Linux with kernel version 3.4.98 was used
in this board. As the GCC compiler available for this board did not support the transactional memory
extension, we had to remove VTMtree from the benchmarks for this platform.


\paragraph{Energy benchmark setup.}

To assess the energy consumption of the trees, energy indicators 
were subsequently collected during 100\% search and 50\% update benchmarks.
The ARM platform was equipped with a built-in "off-chip" power measurement system that 
was able to measure the energy for the A15 cores, A7 cores, and memory in real-time. 
For the Intel HPC platform, a server with two Intel Xeon E5-2690 v2
of 20 cores in total was used. The Intel PCM library using built-in CPU counters was used to measure 
the energy for each CPU and DRAM. 
  
The benchmarks run only with the minimum and maximum
available physical cores. The total energy
consumed by all CPUs and memory (in Joules) was collected and divided by the number of
operations. The collected measurements did not include the initialization cost of trees.


\subsubsection{Performance results.} \label{sec:perfeval}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{\scriptsize\input{figs-uit/perf-4194303}}
\caption{Performance comparison of the tested trees with 
\num[group-separator={,}]{4194303} initial members on an Intel HPC platform with two 8-core chips. On a single chip, the heterogeneous $\Delta$Tree (h$\Delta$Tree) is 140\% faster than the concurrent B-tree (CBTree) in the 50\%-update benchmark with 8 threads. The h$\Delta$Tree performance decreases when the number of threads goes from 8 to 9 because of the cache-coherence issue between two chips (cf. Section \ref{sec:perfeval}).}
\label{fig:perf-4194303}
\end{figure}


\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{\scriptsize\input{figs-uit/perf-2097151}}
\caption{Performance comparison of the tested trees with 
\num[group-separator={,}]{2097151} initial members on an embedded ARM platform. The heterogeneous $\Delta$Tree (h$\Delta$Tree) is 100\% faster than the concurrent B-tree (CBTree) in the 50\%-update benchmark with 4 threads.}
\label{fig:perf-2097151}
\end{figure}

Among the new trees proposed in this paper, b$\Delta$Tree was up to 100\% faster 
than $\Delta$Tree for 100\%
search and was up to 20\% faster in 50\% updates. The h$\Delta$Tree
was up to 5\% faster than b$\Delta$Tree in 100\%
searching. However, in 20\% and 50\% updates,
h$\Delta$Tree was faster by up to 140\% than the b$\Delta$Tree (cf.
Figure \ref{fig:perf-4194303}). 

In comparison with the other trees, Figure 
\ref{fig:perf-2097151} and \ref{fig:perf-4194303} show that the heterogeneous $\Delta$Tree (h$\Delta$Tree)
was the fastest. The h$\Delta$Tree were up to 140\% faster than CBTree
in the 50\% update/8-thread setting on the Intel HPC platform, and  
was up to 100\% faster on the embedded ARM platform
in the 20\% update.  The b$\Delta$Tree's and CBTree's performance was trailing behind h$\Delta$Tree
in all test-cases.

\subsubsection{Energy consumption results.} \label{sec:energyEval}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{x86-power.pdf}}
\caption{Energy efficiency comparison on an Intel HPC platform with two 10-core chips. On a single chip, the heterogeneous $\Delta$Tree (h$\Delta$Tree) was 80\% more energy efficient than the concurrent B-tree (CBTree) in the 50\%-update benchmark with 10 threads. The energy efficiency decreases for some trees in the 50\%-update benchmark with 20 threads (i.e., with 2 chips) because of the cache-coherence issue between two chips (cf. Section \ref{sec:perfeval}). (\textit{Standard errors} $\leq 0.4\%$).}
\label{fig:X86-power}
\end{figure}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{arm-power.pdf}}
\caption{Energy efficiency comparison on an embedded ARM platform. The heterogeneous $\Delta$Tree (h$\Delta$Tree) was 220\% more energy efficient than the concurrent B-tree (CBTree) in the 100\%-search benchmark with 4 threads. (\textit{Standard errors} $\leq 0.27\%$)}
\label{fig:arm-power}
\end{figure}

Among the new trees proposed, balanced $\Delta$Tree (b$\Delta$Tree) was up to 85\% more energy efficient
than $\Delta$Tree (cf. Figure \ref{fig:X86-power}, 100\% search/20-thread setting).
On the other hand, heterogeneous $\Delta$Tree (h$\Delta$Tree) was up to 125\% more energy efficient
than b$\Delta$Tree (cf. Figure \ref{fig:X86-power}, 50\% update/10-thread setting). The results indicated that the 
increased locality by pointer-less $\Delta$Nodes in b$\Delta$Tree and
heterogeneous $\Delta$Nodes with 100\% more leaf nodes in h$\Delta$Tree significantly lowered the energy consumption of the trees.
 
In comparison with the other trees (e.g., CBTree) on the HPC platform (Figure
\ref{fig:X86-power}), h$\Delta$Tree was up to 33\% more energy
efficient in the 100\% search benchmark and 80\% more energy
efficient in the 50\% update/10-thread setting. 

Figure \ref{fig:arm-power} demonstrated the energy efficiency of concurrency-aware vEB-based trees on embedded platform. 
The most energy efficient tree was h$\Delta$Tree which was 
220\% more energy efficient than CBTree and NBBST
in the 100\% search/4-thread setting. In the 50\% update/4-thread setting, 
h$\Delta$Tree was the only one that managed to 
beat CBTree by 180\%.

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{x86-mem-power.pdf}}
\caption{Memory (DRAM) energy consumption on Intel HPC platform. 
Measured using Intel PCM.}
\label{fig:mem-energy}
\end{figure}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{mem-rw-x86.pdf}}
\caption{Amount of data transferred between RAM and CPU for Read + Write operations. Measured using Intel PCM.
Data transfer goes up considerably for some trees in 50\% update
on 20 threads (w/ 2 CPUs) because of the cache-coherence mechanism.}
\label{fig:mem-rw}
\end{figure}

A detailed breakdown of the energy-affecting factors was conducted on the Intel HPC platform.
Figure \ref{fig:mem-energy} shows the DRAM-only energy consumption 
whereas Figure \ref{fig:mem-rw} shows the amount of memory transfers between RAM and CPU for read-write operations.

Figure \ref{fig:mem-rw} shows that h$\Delta$Tree was the 
most efficient in terms of memory transfers between
the RAM and CPU compared to the other trees. 
As a result, h$\Delta$Tree had the lowest DRAM energy 
consumption (cf. Figure \ref{fig:mem-energy}).  

\subsubsection{Energy and performance.}

The experimental results on energy efficiency (Figure
\ref{fig:X86-power} and \ref{fig:arm-power})  and on performance (Figure \ref{fig:perf-4194303} and \ref{fig:perf-2097151}) 
showed that the usage of concurrency-aware vEB layouts 
was able to reduce the $\Delta$Trees' energy consumption and at the same time increase their performance.

If we closely compare side-by-side all of the results on the Intel HPC platform, a strong 
relationship between energy efficiency, performance and data transfer
can be concluded for this platform. As an example, 
in the 100\% search benchmark where concurrency-aware vEB trees are expected
to perform best,  the heterogeneous $\Delta$Tree was 50\% faster 
and 40\% more energy efficient
than CBTree. Figure \ref{fig:mem-rw} tells us that in this scenario, CBTree was transferring
almost $2\times$ more data compared to h$\Delta$Tree. 

However, there are other cases where the energy benefit exceeds 
the performance benefit, which we strongly suspect were attributed
to having a locality-aware data structure.
On the ARM platform, in the 100\% search/4 threads benchmark, 
h$\Delta$Tree was 220\% more energy efficient than 
CBTree while its performance was only 100\% faster.

Figures \ref{fig:perf-4194303} and \ref{fig:X86-power} also show that a less than 2x performance benefit
sometimes results in a 3x to 4x energy benefit for the STM-based trees on the HPC platform. The 
DRAM energy consumption of the STM-based trees
(e.g., AVLtree, RBtree, SFtree and VTMTree) was up to 10x higher than that of the other
trees (cf. Figure \ref{fig:mem-energy}), which partly explains the phenomenon.

Finally, the above evaluation relies to the Intel CPU performance counters or the Intel PCM and ARM
platform off-chip energy counters. Using more robust prediction
models for performance \cite{Chen:2014:EYC:2597479.2597500}
and energy \cite{McCullough:2011:EEM:2002181.2002193} might enable us to 
obtain more
insights that are useful in designing energy-efficient and highly concurrent data structures.

\subsubsection{Multi-CPU coherency issue.} \label{sec:cache-coher}
Figure \ref{fig:perf-4194303} shows some "dips" in performance
for several trees after passing the 8-thread mark on the Intel HPC platform. 
The same behavior was reflected in energy efficiency results (cf. 
Figure \ref{fig:X86-power}). In this chart, the same "dips" were also shown in the 50\% update/20 thread setting. 

Our experimental analysis revealed that these "dips" were caused by the cache coherence protocol in a multi-CPU system. The Intel HPC platform consists of 2 CPUs with 8-cores each. 
Therefore, if a tree
was exploiting data-locality in the cache of a single CPU, cache-coherence protocol did not involve the bus that connects CPUs and memory.  
Starting from 9-threads (or 11-threads in the energy benchmarks), 2 CPUs
were used and therefore the cache-coherence protocol must use the bus to transfer data. 
A closer look at Figure \ref{fig:mem-rw} explains that 
the dips were also related to the increase of RAM-CPU data transfers, which
strengthens the cache-coherence theory.
Moreover, there were no cache-coherence issues 
in the ARM single CPU platform. Therefore, the "dips" did not appeared in any results on the ARM platform.

\subsubsection{Random and sorted inserts.} \label{sec:worstCase}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ 
\begin{tikzpicture}
  \begin{axis}
    [
    width=10cm, height=5cm,
    enlarge y limits=0.2,
    scaled x ticks=false,
    xbar,
    xmin=0,
    xlabel={operations/second},
    symbolic y coords={sorted-insert,random-insert,sorted-search,random-search},
    bar width=6pt,
    ytick=data,
    legend pos=south east
    ]
    
%CBTree
\addplot+  [
	error bars/.cd, 
	x dir=both, 
	x explicit
]
table [x error=error, row sep=crcr] 
{
x        	  y             error \\
2113334.23	sorted-insert 	2888.0704221559\\
1436425.97	random-insert 		2303.2845403101\\
6127972.16	sorted-search 	4352.881447301\\
2495301.85	random-search		4215.9011296083\\
};

%h$\Delta$Tree
\addplot+ [
              	error bars/.cd, 
		x dir=both, 
		x explicit
		]
table [x error=error, row sep=crcr] 
{
x        	y                error \\
2957809.80	sorted-insert  	41063.0593075216 \\
2292632.53	random-insert  		17969.8233327317 \\
9211329.64	sorted-search 	20427.5043253486 \\
3560204.26	random-search 		15008.821675643 \\
};

%std::set
\addplot+ [
              	error bars/.cd, 
		x dir=both, 
		x explicit
		]
table [x error=error, row sep=crcr] 
{
x        	y                error \\
2254212.20	sorted-insert  	52142.1560510366 \\
1500175.49	random-insert		7576.6687994266\\
4482888.90	sorted-search	191164.489145048 \\
1492020.76	random-search		16806.863869775 \\
};

\legend{CBTree, h$\Delta$Tree, std::set}  
\end{axis}
\end{tikzpicture}
}
\caption{Random and sorted insertions/searches of \num[group-separator={,}]{5000000} values on h$\Delta$Tree, CBTree and std::set\textless{int}\textgreater.}
\label{fig:worstcase}
\end{figure}

For $\Delta$Tree, inserting a sequence of increasing (sorted) numbers 
will result in a linked-list of $\Delta$Node.
The bottom-up insertions adopted by balanced $\Delta$Tree and subsequently 
heterogeneous $\Delta$Tree was supposed to prevent this (worst-case) from happening.

Therefore, we tested CBTree and h$\Delta$Tree for random and sorted number insertions. 
GCC standard library std::set\textless{int}\textgreater was also included as a baseline. For the sorted
inserts, 
starting with a blank tree, an increasing sequence of \num[group-separator={,}]{5000000} 
numbers starting from 1 were inserted into the tree using a single thread. The
same amount of random numbers was used instead for the random inserts. 
These tests were done on the same HPC platform described in Section \ref{sec:benchsetup}.
Since std::set currently not supporting
concurrent operations, concurrent insert test was deliberately left out.

The result in Figure \ref{fig:worstcase} showed that h$\Delta$Tree was 38\% faster than 
CBTree and 30\% faster than std::set in the sorted inserts. 
For random inserts, the h$\Delta$Tree was about 50\%
faster compared to CBTree and std::set. Further evaluation with \textit{perf} revealed
that in h$\Delta$Tree, random inserts triggers more branch misses (6.82\%) compared
to sorted inserts (1.04\%).

We also measured the time required to search all of the inserted values 
using the same way as they were inserted (random or sorted). 
In Figure \ref{fig:worstcase}, h$\Delta$Tree was up to 105\% faster in the random search
compared to std::set. This lead was increased to 130\% 
when searching the sorted sequence of inserted numbers.

The above results means two things: 1) h$\Delta$Tree performed better in both of the worst and average
case of tree search/update compared to optimized B-tree and the widely used std::set; 
and 2) random value inserts and searches were not actually
benefit the B-tree based tree. Therefore, the benchmark setups
in Section \ref{sec:benchsetup} is assured to give a fair comparison of all the tested trees
performance.

\paragraph{Performance with different upper-bound UB.} \label{sec:diff-UB}

\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ 
\begin{tikzpicture}
\begin{axis}
[
		ylabel={operations/second},
		ymin = 2500000,
		ymax = 5000000,
		scaled y ticks=false,
		width=10cm, height=3.5cm, enlarge y limits=0.5,
		xlabel={$\UB$ (in KB)},
		xmin = 4,
		xmax = 2048,
		symbolic x coords={4, 8, 16, 32, 64, 128, 256, 512, 1024, 2048, 16182, 32364, 65728},
		xtick=data,
		legend pos=north east
]
\addplot+ [
	blue,
	mark=none,
	error bars/.cd, 
	y dir=both, 
	y explicit
]
table [y error=error, row sep=crcr] 
{
x        	y                               error \\
4       	5280388.63660365   14974.8632430073\\
8       	5275931.20185713   10513.7949942302\\
16     	5069451.48534929   13717.0176713126\\
32     	4836993.32494921  	 21505.5609672388\\
64     	4540088.98574412    12451.1380904163\\
128   	4211235.57651815   9011.8899618601\\
256		3790750.56861259	14209.2285225684\\
512		3344257.90916996   28085.6294077072\\
1024  	2918344.71487772  36124.9734022401\\
2048 	2123683.31634387   35077.1012163309\\
16182	2237837.35398111  42556.6143950982\\
32364	3227680.58872894	58070.6098121757\\
65728	3804885.47294726	62555.1530207667\\
};

\addplot+ [
	red,
	mark=none,
	error bars/.cd, 
	y dir=both, 
	y explicit
]
table [y error=error, row sep=crcr] 
{
x        	y                                 error \\
4       	2726132.70814023   51932.6296177883\\
8       	2913413.35508682   126203.915659568\\
16     	2749670.03959525   115801.576270052\\
32     	2684852.06465124   122482.151211992\\
64     	2788622.42052426     169185.435791652\\
128   	2742280.48044754   107577.6197528\\
256   	2832700.69684437   170819.544797631\\
512   	2832700.69684437  	181871.407518969\\
1024 	2843332.38555587   188067.455580507\\
2048 	2954209.74889217  	222482.331581449\\
16182 	3023705.85389453	212111.49130874\\
32364	3086419.75308642	196655.1752026\\
65728	3119800.3327787	7867.2148088397\\
};
\legend{10\% update, 100\% search}
\end{axis}
\end{tikzpicture}
}
\caption{Performance of the 100\%-search and 10\%-update benchmarks using different upper bounds $\UB$, which was evaluated on an Intel HPC platform. The system page size was 4KB. Note that the $x$-axis uses a log-scale.}
\label{fig:diff-UB}
\end{figure}

Concurrency-aware vEB layout required that an upper-bound $\UB$ to be specified in advance; and 
thus, one would argued that $\UB$ is a fine-tuneable aspect that could determine 
the performance of the concurrency-aware vEB trees. 
To prove that this is not the case, we tested the Heterogeneous
$\Delta$Tree (h$\Delta$Tree) using different upper-bound $\UB$ values, 
starting from 4KB (small page size) up to 2MB (huge page size) using
single thread. 

We tested two cases, 100\% search and 10\% update 
(90\% Search, 9\% Insert, and 1\% Delete) operations.
For the 100\% search test, this tree was initially filled with $(2^{22} -1)$ random values 
and times were recorded to conduct 5 million operations of 100\% search.
For 10\% update test, starting from empty tree, we conducted 5 million operations of
90\% search, 9\% insert and 1\% delete operations. These update parameters
was based on the (anecdotal) evidence of the method call distribution of sets
\cite{Herlihy:2008:AMP:1734069}.

The heterogeneous $\Delta$Tree was shown to be resilient to different upper-bound $\UB$ (cf. Figure \ref{fig:diff-UB}).
This was an expected result according to Lemma \ref{lem:dynamic_vEB_search}. In fact, $\UB$ can
be as big as the whole tree and searching performance is still going to be optimal, provided the meta-data 
(e.g., the tree map in Section \ref{sec:mapdesc}) occupied only a small fraction of the LLC.
As mentioned in Section \ref{sec:relaxed-veb}, small $\UB$ benefits only the concurrent tree updates.

\subsubsection{$\Delta$Tree memory usage.}

The $\Delta$Trees method of only marking nodes for deletion will not results in memory leaks 
or generating plenty of wasted memory that might affect the 
trees performance.
Maintenance operations (e.g., Rebalance, Expand, Split and Merge) perform also the garbage
collection, eliminating the marked nodes.
$\Delta$Trees do not pre-allocate memory for $\Delta$Nodes nor their mirrors. A $\Delta$Node consists of
several basic nodes in the vEB layout. Memory for each $\Delta$Node and its mirror was
dynamically allocated on demand at $\Delta$Node creation.

In practice, the actual size of the heterogeneous $\Delta$Tree with 4.2 million keys
(giving memory footprint of 97.9 MB) was 32\% less than that of CBTree (giving memory
footprint of 143 MB) since the former uses Map (Section \ref{sec:mapdesc}) instead of pointers.
This claim is also supported by Figure \ref{fig:mem-rw} in which $\Delta$Trees were efficient in terms of data transfers between RAM and CPU, even in the 50\% update cases where deletions made up 25\% of the whole operations.

\subsubsection{Caching and branching evaluation.} \label{sec:cache-branch}

The use of map instead pointers and keeping the tree balanced
has managed to lower the cache-misses of b$\Delta$Tree by 40\% compared to $\Delta$Tree. 
Heterogeneous leaf $\Delta$Nodes that can hold
twice many keys were managed to lower the search time and $\Delta$Nodes' rebalance overheads.
It was also shown h$\Delta$Tree was having up to 30\% less cache-misses 
and 20\% more efficient branching than b$\Delta$Tree because of the heterogeneous leaf $\Delta$Nodes.  

The CBTree layout, 
although fast and highly-concurrent, suffered from
high branching operations. CBTree
branching was up to 90\% more of that b$\Delta$Tree and h$\Delta$Tree. Its cache references
were also 150\% higher than b$\Delta$Tree and h$\Delta$Tree, as expected in B-tree 
since block $B$ is not optimal for transfers between the memory levels.

Unix's \textit{perf} was used to measure the cache and branch profiles using the Intel HPC platform.

% END SECTION


==> Deliverable-Contributions-before-merging.tex <==
The main achievements of this report are summarized in two main parts as below.

\paragraph{White-box methodologies} provides the cache-oblivious methodology and energy models.
\begin{itemize}
\item We have devised a new {\em relaxed} cache oblivious model and a novel {\em
  concurrency-aware} vEB layout that makes the vEB layout suitable for highly-concurrent 
  data structures with update operations (cf. Figure \ref{fig:dynamicVEB}). The concurrency-aware vEB layout supports
  dynamic node allocation via pointers while maintaining the optimal search 
  cost of $O(\log_B N)$ memory transfers without knowing the exact value of block size $B$
  (cf. Lemma \ref{lem:dynamic_vEB_search}). 
\item We have proposed an energy model which is able to predict the power consumed by a program running on a specific number of cores. Given a certain platform and the computation intensity, the model can predict the power consumed by a computational algorithm, then help to answers the question how many cores are required to run a program to achieve the optimized energy consumption. The model considers both platform and algorithm properties which give more insight on how to design the algorithm to achieve better energy optimization. The model is also validated the model with a set of micro-benchmarks and real applications such as  sparse/dense linear algebra kernels and the graph computation algorithm. 
\item We have continued the work done in D2.1~\cite{EXCESS:D2.1} on the modeling of
queue implementations. We have moved from a grey-box
model, where the performance and the power consumption of enqueue and
dequeue operations were hidden, to a white-box model, where the impact
of those operations are studied separately, and combined at the
end. Additionally, we have generalized the model to offer more
freedom according to the workers calling the \ds (parallel section
sizes of enqueuers and dequeuers are decoupled);
\end{itemize}

\paragraph{Libraries and programming abstractions} provides a set of implemented concurrent search trees and their energy and performance analyses,
as well as a set of implemented lock-free queues, together with a comparison between the predicted and measured throughput and power. 
\begin{itemize}
\item We have developed the concurrent search tree libraries package that contains several state-of-the-art concurrent search trees such as the non-blocking binary search tree, the Software Transactional Memory (STM) based red-black tree, AVL tree, and speculation-friendly tree, the fast concurrent b-tree, and the static cache-oblivious binary search tree. A family of novel locality-aware and energy efficient concurrent search trees, namely the DeltaTree, the Balanced DeltaTree, and Heterogeneous DeltaTree are also enclosed in the concurrent search tree libraries package. All the components in this package support the stand-alone benchmark program mode for the purpose of micro-benchmarking and library mode that is pluggable into any C/C++ based programs.
\item The DeltaTrees are platform-independent and up to 140\% faster and 220\% more energy efficient than the state-of-the-art on commodity HPC and embedded platforms. In single thread evaluation, Heterogeneous DeltaTree is 38\% faster than B-tree based STD::Set of GCC standard library in the theoretical worst-case scenario of inserting a sorted sequence of keys; and is 50\% faster than STD::Set for inserting a random sequence of keys — the theoretical average-case scenario.
\item On this side, compared to D2.1~\cite{EXCESS:D2.1}, we have automatized the process of estimating the performance and the
  power consumption and integrated it in the EXCESS software.
\end{itemize}
This report is organized as follows. Section 2 is the description of EXCESS platforms and their setting to measure the energy consumption. The white-box methodology such as cache-oblivious model and algorithms are described detailed in section 3. Section 4 is the proposed energy model and its evaluated with both micro-benchamarks and application benchmarks. Section 5 is the first prototype of EXCESS libraries and programming abstractions such as numerous concurrent search tree implementations and their performance and energy analyses. Section 6 discusses the findings and future works of this study. 


==> Energy-Model-Motivation.tex <==
The great amounts of energy consumed by worldwide computing systems increase 7\% annually and becomes a major concern in information technology society. In order to tackle this issue, the research community and industry have proposed several research approaches  to reduce the energy consumption of IT systems \cite{Orgerie2014}.

One of the key research directions to improve energy-efficiency is to understand how much energy a computing system consumes and characterize the power consumed by individual components. By knowing the energy consumption of an algorithms on a specific computing architecture, researchers and practitioners can design and implements new approaches to reduce the energy consumed by a specific platform of a certain algorithm.

The energy consumption of computing systems can be either measured by energy sensors and external energy-meter equipment or estimated by energy models. Energy measurement equipment and energy sensors are not always available and can be costly to deploy and set up. Therefore, energy model is an alternative and less expensive way to estimate the energy consumption of a computing components or a whole computing system. The energy models, however, need to be simple to use and should not interfere with the energy estimated results \cite{Orgerie2014}.

The objective of this study is to build a energy model that can estimate the energy consumption of an algorithm on a given platform. In order to do so, the model consider both algorithmic and platform properties. Our model is inspired by "Amdahl" law analysis and the roofline model of energy \cite{Choi:2013:RME:2510661.2511392}, \cite{6877278}. The roofline model also connect algorithmic and platform properties but does not consider the number of cores as a parameter. By estimating the power consumed by a system running a specific number of cores, our model can predict the number of cores required to achieve the least energy consumption. 

One of the most popular strategy to reduce the energy consumption is race-to-halt strategy \cite{Awan:2011:ERL:2056313.2056722}. This strategy assumed that the system should run as fast as possible and then go to sleep to save energy. For new and high energy-efficient platforms which has significant low static power, race-to-halt might not be always true. As far as we know, there is no study yet showing the real scenario that race-to-halt is not always applicable. In our model, we target to predict when race-to-halt is not applicable and analyze the trade-off between the performance and energy efficiency. We also present an application scenario when race-to-halt no longer works. 

==> executive-summary-before-merging.tex <==
Computing technology is currently at the beginning of the disruptive transition from petascale to exascale computing (2010 –- 2020), posing a great challenge on energy efficiency. High performance computing (HPC) in 2020 will be characterized by data-centric workloads that, unlike those in traditional sequential/parallel computing, are comprised of big, divergent, fast and complex data. In order to address energy challenges in HPC, the new data must be organized and accessed in an energy-efficient manner through novel fundamental data structures and algorithms that strive for the energy limit. Moreover, the general application- and technology-trend indicates finer-grained execution (i.e. smaller chunks of work per compute core) and more frequent communication and synchronization between cores and uncore components (e.g. memory) in HPC applications. Therefore, not only concurrent data structures and memory access algorithms but also synchronization is essential to optimize the energy consumption of HPC applications. However, previous concurrent data structures, memory access algorithms and synchronization algorithms were designed without energy consumption in mind. The design of energy-efficient fundamental concurrent data structures and algorithms for inter-process communication in HPC  remains a largely unexplored area and requires significant efforts to be successful.

Work package 2 (WP2) aims to develop interfaces and libraries for energy-efficient inter-process communication and data sharing on the new EXCESS platforms integrating Movidius embedded processors. In order to set the stage for these tasks, WP2 needs to investigate and model the trade-offs between energy consumption and performance of data structures and algorithms for inter-process communication. 
WP2 also concerns supporting energy-efficient massive parallelism through scalable concurrent data structures and algorithms that strive for the energy limit, and minimizing inter-component communication through locality- and heterogeneity-aware data structures and
algorithms.

The early result of Task 2.2 (PM7 - PM36) on white-box methodology and modeling the consumed energy of concurrent data structures and algorithms, as available by project month 18, are summarized in this report. 

\paragraph{White-box methodologies} provides the cache-oblivious methodology and energy models.
\begin{itemize}
\item We have devised a new {\em relaxed} cache oblivious model and a novel {\em
  concurrency-aware} vEB layout that makes the vEB layout suitable for highly-concurrent 
  data structures with update operations (cf. Figure \ref{fig:dynamicVEB}). 
\item We have proposed an energy model which is able to predict the power consumed by a program running on a specific number of cores. We validate the model with a set of micro-benchmarks and real applications such as  sparse/dense linear algebra kernels and the graph computation algorithm. The model can support the prediction of when to apply race-to-halt strategy and give examples when race-to-halt is no longer applicable for the energy optimization.
\item We have propose a way to model the energy behavior of
lock-free queue implementations and parallel applications that use
them, on CPU platforms. Focusing on steady state behavior we decompose
energy behavior into throughput and power dissipation which can be
modeled separately and later recombined into several useful metrics,
such as energy per operation.
\end{itemize}

\paragraph{Libraries and programming abstractions} provides a set of implemented concurent search trees and their energy and performance analyses.
\begin{itemize}
\item We have developed the concurrent search tree libraries package that contains several state-of-the-art concurrent search trees such as the non-blocking binary search tree, the Software Transactional Memory (STM) based red-black tree, AVL tree, and speculation-friendly tree, the fast concurrent b-tree, and the static cache-oblivious binary search tree. A family of novel locality-aware and energy efficient concurrent search trees, namely the DeltaTree, the Balanced DeltaTree, and Heterogeneous DeltaTree are also enclosed in the concurrent search tree libraries package.
\item The DeltaTrees are platform-independent and up to 140\% faster and 220\% more energy efficient than the state-of-the-art on commodity HPC and embedded platforms. 
\item On lock-free queues on CPU platforms, we have automatized the process of estimating the performance and the power dissipation of any queue implementation, and integrated it in the EXCESS software.
\end{itemize}

